PresAIse, A Prescriptive AI Solution for Enterprises

Prescriptive AI represents a transformative shift in decision-making, offering causal insights and actionable recommendations. Despite its huge potential, enterprise adoption often faces several challenges. The first challenge is caused by the limitations of observational data for accurate causal inference which is typically a prerequisite for good decision-making. The second pertains to the interpretability of recommendations, which is crucial for enterprise decision-making settings. The third challenge is the silos between data scientists and business users, hindering effective collaboration. This paper outlines an initiative from IBM Research, aiming to address some of these challenges by offering a suite of prescriptive AI solutions. Leveraging insights from various research papers, the solution suite includes scalable causal inference methods, interpretable decision-making approaches, and the integration of large language models (LLMs) to bridge communication gaps via a conversation agent. A proof-of-concept, PresAIse, demonstrates the solutions' potential by enabling non-ML experts to interact with prescriptive AI models via a natural language interface, democratizing advanced analytics for strategic decision-making.

==> user-experience-walkthru.tex <==
In observation of our user design principles as described in section \ref{subsect_user_experience_principles},
we have implemented a user experience web application which integrates a conversation
agent with a high fidelity dashboard as would be commonly used in business intelligence (BI)
and analytics settings.



The user experience is a concatenation of two sub-experiences:

\begin{itemize}
    \item A conversational dialog area that captures the overall dialog between the user and the conversational agent
    in a streaming textual format. Note that we have structured the dialog area to resemble a chat session
    or a text interchange on a mobile device.
    The dialog area has the following types of components:
    \begin{itemize}
        \item Textual user inputs (seen in blue). These can be modified in the future to handle translated speech.
        \item Textual responses from the language model (see in the white responses). These responses can be
        used to acknowledge that the agent has completed a requested task, explain why a task failed,
        or ask for additional information or clarification if user requests are insufficient.
        \item Textual summaries of task outputs. In our case, these are summarizations of key performance indicators
        when the user task is to engage an optimization model.
    \end{itemize}

    \item A traditional business intelligence (BI) dashboard area. The dashboard area contains three components:
    \begin{itemize}
        \item Parameter capture area that summarizes the inputs to and underlying causal reasoning model, in this case
    capturing the origin and destination cities which define a pricing market.
        \item A key performance indicator (KPI) area that summarizes the performance of underlying optimization models
        as applied to known historical customer data.
        Notice that in this particular domain the KPIs specify revenue uplift, which is the additional revenue that can
        be expected if the displayed pricing strategy is put into place, and the conversion rate, which is the percent of
        customers which are expected to purchase the underlying product (travel tickets) at the improved prices.
        \item A policy summary area that indicates pricing rules as applied to various strategies for segmenting the
        customer space.
    \end{itemize}
    
\end{itemize}

Figure \ref{fig:intro-screen-shot} displays the user experience after an introductory level of dialog. Here the user is requesting
a historical analysis of the pricing policies as seen in an underlying historical pricing data set.
Notice that the conversational agent deems the initial request from the user (``Can you show me the base pricing policy")
does not specify the travel market and is insufficient to provide a reasonable response. 
Thus the agent constructs a response that prompts the user to input an origin and destination city pair.
This illustrates one of the powers of the conversational style of dialog in that the user is prompted for
more information in a natural form (compare this to an intrusive error dialog in a traditional interactive user experience).

Once the user provides the requested parameters, the underlying historical analysis is runnable, indicating that the
base price (``full fare") for the market is \$510. Note that the conversational dialog is augmented with a summary
of the performance when this price is applied, summarizing the average upsell revenue per booking and the conversion rate.



Note that in general a text only interaction is ``not-enough" for completing complicated analytical or business intelligence (BI) tasks. However, BI-style dashboards are often ``too much" for non-expert users who may not be expert in data science or machine learning. There is a need for easily interpreting what the non-expert user is trying to accomplish yet to offer that user
some of the power afforded by expert interfaces.
It is natural to aim for a design goal which simply bolts one onto the other.
We have aimed for a more refined goal which adds capabilities to a text-only chat interaction and
uses some of the capabilities of the more advanced type experience to cue the user about what is next.

In our example application the "what is next" cues are provided by our pricing grid, which lead the user through a process
of filling in the blanks. The grid, for example, displays three potential dimensions along which pricing rules may
be customized:

\begin{itemize}
    \item Stay Restrictions.
    \item Fare Discount Levels.
    \item Advance Purchase Windows.
\end{itemize}

The user is able to request increased or decreased levels of granularity of the subdivisions in this pricing grid.
The user can then ask for various levels of refinement of these policies by asking for optimizations to be applied.

Figure \ref{fig:single-rule-screen-shot} illustrates a pricing policy in which a single AI-generated pricing rule is applied to
all potential customer segments. This pricing rule determines that performance is improved by lowering the offered
base prices from \$510 to \$475. This results in an increase of conversions (sales) from 5.2\% to 6.1\% and an
overall increase in revenue by 1.5\% (more sales at a lower price).

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/AIGeneratedSinglePolicyScreenShot.png}
    \caption{Single Rule AI Generated Pricing Policy Screen}
    \label{fig:single-rule-screen-shot}
\end{figure}

Notice that the pricing grid is still somewhat barren. Contrary to traditional user design mantras, we have found
that empty space can help to guide or motivate the user toward the next level of exploration.
As illustrated in Figure \ref{fig:2-rule-screen-shot} for example, the user can request that additional pricing rules
be generated which segment the user space into two distinct rules -- note that the optimization model generated two
pricing rules which raises the price for full fare customers to \$635 dollars and lowers the price for
discounted customers to \$445.
The user can continue to segment the customer population -- Figure \ref{fig:18-rule-screen-shot}  gives and example of asking for a maximal segmentation of
customers into 18 different pricing groups.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/AIGenerated2RulePolicyScreenShot.png}
    \caption{Two Rule AI Generated Pricing Policy Screen}
    \label{fig:2-rule-screen-shot}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/AIGenerated18RulePolicyScreenShot.png}
    \caption{Maximally Differentiated AI Generated Pricing Policy Screen}
    \label{fig:18-rule-screen-shot}
\end{figure}

The user can ask for additional refinements of the pricing policies, for example, specifying
minimum and maximum pricing bounds (these are considered ``counterfactual" or ``what-if") types of
tasks in that they can ask the models to institute pricing policies that are speculative and are not seen in
historical data sets.

==> user-experience.2023-11-30.tex <==
\subsection{Integrating a High Fidelity User Experience with a Large Language Model}

A key challenge in our solution is to provide a high fidelity user experience for the
causal problem solving process that integrates language model interactions with a user
experience that is natural and useful to the end user.

Several particular problems arise. The first regards state.
Modern language models incorporate capabilities for managing state, which affords
multi-step interactions which have found great success
in conversational systems such as ChatGPT.
In chat oriented systems the concept of state is generally clear -- it is the collection
of prior inputs from the user coupled with the prior responses from the language model.
However, with more advanced solutions such as that offered by the present work,
it is not always clear to the user what the state of the language model is.
This lack of clarity is often amplified as the user progresses through a multi-stage problem solving process.
Thus, our solution attempts to emphasize state.

A second challenge is to provide a user experience which is goal oriented.
Again, we contrast our solution with chat-oriented conversational systems.
Line-of-business problem solving interactions are often done with a clear outcome or goal.
For example, the goals may be to:

\begin{itemize}
    \item Establish a domain of investigation or operation. For example, the system
    would want to establish which market or geography the user has in mind in a marketing/pricing application.
    \item Establish parameters for solutions or optimization processes.
    \item Set bounds on the complexity of the solution process,
    For example, in performing causal analyses, the user will often want to reduce
    the underlying dimensionality of the system, or to limit the number of covariates to be investigated.
    \item Set constraints or boundary conditions.
    For example, what are the minimum and maximum prices for a pricing strategies.
    How many customer groups or segments should be considered?
    \item Choose an analytical method to employ. Should the interaction trigger a full scale
    optimization, should it simply perform a historical analysis, etc.
    \item Initiate counterfactual ("what-if") investigations.
\end{itemize}

In some cases the system will have certain parts of the process which are prerequisite to the others.
The conversational agent should be aware of this as it "directs" the conversation -- an attribute
of the system which is especially pronounced in importance for inexperienced users.

Keeping in mind these challenges and in pursuit of the main goals (1), (2) and (3) outlined in the
introductory section, we have designed our user experience with the following
concrete objectives in mind:

\begin{itemize}
    \item The conversational state and history of the language model should be incorporated into the
    user experience as a first class element.
    \item Information that is gathered conversationally from the user should be displayed to the user,
    making clear the internal state of the language model.
    \item Cues should be provided within the user experience about information that is yet to be gathered
    from the user,
    \item Cues should be given within the user experience about potential future interactions and capabilities
    that can achieved via the language model.
    \item Alteration of the graphical user experience can be used to guide the conversation.
    \item Provide active cues which signal changes in the causal model as the conversation proceeds.
\end{itemize}

We illustrate these principles in the user experience seen in Figure \ref{fig:intro-screen-shot}.
This user experience is geared toward a line-of-business user in the travel industry.
who is seeking to analyze pricing
strategies as applied to various sales regions or sub-markets.
As the user is NOT a data scientist, the user experience is centered around more familiar concepts
such as a pricing table.

The user experience is a concatenation of two sub-experiences:

\begin{itemize}
    \item A conversational dialog area that captures the overall dialog between the user and the conversational agent
    in a streaming textual format. Note that we have structured the dialog area to resemble a chat session
    or a text interchange on a mobile device.
    The dialog area has the following types of components:
    \begin{itemize}
        \item Textual user inputs (seen in blue). These can be modified in the future to handle translated speech.
        \item Textual responses from the language model (see in the white responses). These responses can be
        used to acknowledge that the agent has completed a requested task, explain why a task failed,
        or ask for additional information or clarification if user requests are insufficient.
        \item Textual summaries of task outputs. In our case, these are summarizations of key performance indicators
        when the user task is to engage an optimization model.
    \end{itemize}

    \item A traditional business intelligence (BI) dashboard area. The dashboard area contains three components:
    \begin{itemize}
        \item Parameter capture area that summarizes the inputs to and underlying causal reasoning model, in this case
    capturing the origin and destination cities which define a pricing market.
        \item A key performance indicator (KPI) area that summarizes the performance of underlying optimization models
        as applied to known historical customer data.
        Notice that in this particular domain the KPIs specify revenue uplift, which is the additional revenue that can
        be expected if the displayed pricing strategy is put into place, and the conversion rate, which is the percent of
        customers which are expected to purchase the underlying product (travel tickets) at the improved prices.
        \item A policy summary area that indicates pricing rules as applied to various strategies for segmenting the
        customer space.
    \end{itemize}
    
\end{itemize}

Figure \ref{fig:intro-screen-shot} displays the user experience after an introductory level of dialog. Here the user is requesting
a historical analysis of the pricing policies as seen in an underlying historical pricing data set.
Notice that the conversational agent deems the initial request from the user ("Can you show me the base pricing policy")
does not specify the travel market and is insufficient to provide a reasonable response. 
Thus the agent constructs a response that prompts the user to input an origin and destination city pair.
This illustrates one of the powers of the conversational style of dialog in that the user is prompted for
more information in a natural form (compare this to an intrusive error dialog in a traditional interactive user experience).

Once the user provides the requested parameters, the underlying historical analysis is runnable, indicating that the
base price ("full fare") for the market is \$510. Note that the conversational dialog is augmented with a summary
of the performance when this price is applied, summarizing the average upsell revenue per booking and the conversion rate.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/IntroScreenShot.png}
    \caption{Introductory Screen}
    \label{fig:intro-screen-shot}
\end{figure}

Note that in general a text only interaction is "not-enough" for completing complicated analytical or business intelligence (BI) tasks. However, BI-style dashboards are often "too much" for non-expert users who may not be expert in data science or machine learning. There is a need for easily interpreting what the non-expert user is trying to accomplish yet to offer that user
some of the power afforded by expert interfaces.
It is natural to aim for a design goal which simply bolts one onto the other.
We have aimed for a more refined goal which adds capabilities to a text-only chat interaction and
uses some of the capabilities of the more advanced type experience to cue the user about what is next.

In our example application the "what is next" cues are provided by our pricing grid, which lead the user through a process
of filling in the blanks. The grid, for example, displays three potential dimensions along which pricing rules may
be customized:

\begin{itemize}
    \item Stay Restrictions.
    \item Fare Discount Levels.
    \item Advance Purchase Windows.
\end{itemize}

The user is able to request increased or decreased levels of granularity of the subdivisions in this pricing grid.
The user can then ask for various levels of refinement of these policies by asking for optimizations to be applied.

Figure \ref{fig:single-rule-screen-shot} illustrates a pricing policy in which a single AI-generated pricing rule is applied to
all potential customer segments. This pricing rule determines that performance is improved by lowering the offered
base prices from \$510 to \$475. This results in an increase of conversions (sales) from 5.2\% to 6.1\% and an
overall increase in revenue by 1.5\% (more sales at a lower price).

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/AIGeneratedSinglePolicyScreenShot.png}
    \caption{Single Rule AI Generated Pricing Policy Screen}
    \label{fig:single-rule-screen-shot}
\end{figure}

Notice that the pricing grid is still somewhat barren. Contrary to traditional user design mantras, we have found
that empty space can help to guide or motivate the user toward the next level of exploration.
As illustrated in Figure \ref{fig:2-rule-screen-shot} for example, the user can request that additional pricing rules
be generated which segment the user space into two distinct rules -- note that the optimization model generated two
pricing rules which raises the price for full fare customers to \$635 dollars and lowers the price for
discounted customers to \$445.
The user can continue to segment the customer population -- Figure \ref{fig:18-rule-screen-shot}  gives and example of asking for a maximal segmentation of
customers into 18 different pricing groups.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/AIGenerated2RulePolicyScreenShot.png}
    \caption{Two Rule AI Generated Pricing Policy Screen}
    \label{fig:2-rule-screen-shot}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/AIGenerated18RulePolicyScreenShot.png}
    \caption{Maximally Differentiated AI Generated Pricing Policy Screen}
    \label{fig:18-rule-screen-shot}
\end{figure}

The user can ask for additional refinements of the pricing policies, for example, specifying
minimum and maximum pricing bounds (these are considered "counterfactual" or "what-if") types of
tasks in that they can ask the models to institute pricing policies that are speculative and are not seen in
historical data sets.
